Imaginary Machines: A Serverless Model for Cloud Applications

Serverless Function-as-a-Service (FaaS) platforms provide applications with resources that are highly elastic, quick to instantiate, accounted at fine granularity, and without the need for explicit runtime resource orchestration. This combination of the core properties underpins the success and popularity of the serverless FaaS paradigm. However, these benefits are not available to most cloud applications because they are designed for networked virtual machines/containers environments. Since such cloud applications cannot take advantage of the highly elastic resources of serverless and require run-time orchestration systems to operate, they suffer from lower resource utilization, additional management complexity, and costs relative to their FaaS serverless counterparts. We propose Imaginary Machines, a new serverless model for cloud applications. This model (1.) exposes the highly elastic resources of serverless platforms as the traditional network-of-hosts model that cloud applications expect, and (2.) it eliminates the need for explicit run-time orchestration by transparently managing application resources based on signals generated during cloud application executions. With the Imaginary Machines model, unmodified cloud applications become serverless applications. While still based on the network-of-host model, they benefit from the highly elastic resources and do not require runtime orchestration, just like their specialized serverless FaaS counterparts, promising increased resource utilization while reducing management costs.

==> implementation.tex <==
\newpage
\clearpage

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/IM-many-plats.pdf}
  \caption{Platform support for IM model: native (left) vs IM-over-FaaS (right).}
  \label{fig:many-plats}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/IM-states.pdf}
  \caption{IM-over-FaaS Host Function states}
  \label{fig:states}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/IM-node.pdf}
  \caption{IM-over-FaaS Host Function instance control and data channels}
  \label{fig:channels}
\end{figure}

\section{Realizing Imaginary Machines}

\begin{enumerate}

    \item Ideally this model would be provided by a serverless platfrom (that could possibly provided multiple programming models)
    
    \item Although the implementation is less straightforward without privileged control of the platform. We are building a prototype using publicly available FaaS platform to be able to run unmodified off-the-shelf cloud applications on AWS Lambda without the need for orchestration. IM-over-FaaS.
    
    \item We are extending a system that already provides a network-of-hosts model on top of AWS Lambda and is capable of running unmodified cloud applications. The system can run cloud applications on the serverless platform, however, it requires an explicit serverfull orchestration system at runtime. In some of the use cases, it relied on a docker-compose orchestrator, which goes against the Imaginary Machines model of not requiring an explicit run-time orchestrator. 

    \item --
    \item We refer to networked functions with assigned addresses and hostnames as hosts. 
    \item --
    \item hostnames and IP addresses assigned to particular function instances
    \item function instances started on the first network communication addressing them
    \item function instances suspended if idle and resumed on new communication requests and timers
    \item unexpected function cold starts are treated as host faults followed by restart.
    \item --
    \item Only static-time system configuration is required -- including registering the functions with the FaaS service and providing a mapping between hostname patterns and FaaS function names.
    
    \item We are extending it to provide the necessary mechanisms to perform transparent run-time orchestration of AWS Lambda function to provide the Imaginary Machines serverless model.
    
    \item The system intercepts application control stream socket connection requests to provide networking to the application processes running in AWS Lambda.
    \item We are leveraging this intercepted application signal as the possible 

    \item The system intercepts all socket control operations and keeps track of the application socket state. 
    
    \item These signals are sufficient to build an initial support a simplified Imaginary Machines, that does cover all of the cases, but will be sufficient to support many common cloud applications.
    
    \item Some signals are not recoverable in an unprivileged IM-over-FaaS implementation (but easily visible in an IM-native implementation), introducing an additional mechanism.
    For example, if a host function has an open connection to an external host, once the function is suspended, the signaling of the arrival of new data on the external connection is not available to intercept.
    The most conservative strategy is not to suspend functions that depend on externally generated signals. This strategy implies that applications with idle external connections would keep host functions running. 
    Another extreme is to consider host functions with idle external connections as preemptible, possibly forcing applications to consider such connections as lost and required to be reestablished if needed again. There is a large space of options in between, including keeping host functions warm for a certain time, introducing network canary intermediaries, and further distinguishing strategies based on whether the host function was an active or a passive endpoint of the external connection. 
    
    
    \item The signal to establish a connection to a remote host is intercepted, and before the connection is established, based on the state of the destination host, an orchestration action may need to be performed.

    \begin{enumerate}
        \item If the destination host is in \texttt{running} state, the connection setup proceeds as usual. 
        \item If the destination host is in \texttt{sleeping} state, the function manager is instructed to resume the destination host, and only once the host is in \texttt{running} state the connection setup proceeds.
        \item If the destination host is in \texttt{terminated} state, connection failure is signaled to the application.
        \item Otherwise, if the destination address can be mapped to a valid function type, the host is instantiated, and once it is in \texttt{running} state the connection continues.
    \end{enumerate}

    \item When the application processes running on a host are idle and do not have any established connections, the host is suspended and enters \texttt{sleeping} state. The host is then periodically resumed by the function manager to keep it warm and give the application the opportunity to handle any timer-like events that may trigger further processing and resume the function into \texttt{running} state. 
    Note that this is a simplified version of the 

    \item When the application processes stop, either by exiting or due to a fault, the function is \texttt{stopped}, and its resources are released.
    

    
\end{enumerate}

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/IM-mMV-lifecycle.pdf}
  \caption{[OLD] IM-microVM lifecycle}
  \label{fig:lifecycle}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=1\linewidth]{figures/boxer-node-dreamer.pdf}
  \caption{[OLD] Boxer-IM node}
  \label{fig:boxer-im-node}
\end{figure}


\ana{Attempt of the intro storyline based on what we discussed:}

\begin{itemize}
    \item Cloud users today can choose between two main options for developing and managing their applications: renting VMs on-demand or using providers' serverless compute and storage services. VMs come with a familiar programming/execution environment of a network of hosts but users need to explicitly turn machines on/off based on the application load. Serverless automates infrastructure management, but comes with a restrictive programming model (e.g., FaaS). 
    \item In this paper, we explore how to get the best of both worlds. We explore how to automate infrastructure orchestration à la serverless, but for VM-based workloads with the familiar network-of-hosts programming/execution model. We observe that the infrastructure orchestration that serverless platforms provide involves capturing workload invocation and termination signals and triggering machines to turn on or off. While today's serverless platforms capture these signals by requiring users to express their applications in a new event-based programming model, we propose to achieve the same in conventional VM-based applications by capturing system calls. For example, the cloud infrastructure can take action to boot a server when detecting a client application issuing a connect syscall. 
    \item We propose a unified model of cloud computing, which we call \textit{imaginary machines}, that preserves the familiar, well-loved network-of-hosts programming model of VM-based applications with the orchestration automation of serverless platforms. We propose to implement this with an interposition layer that intercepts system calls in applications and automatically launches and terminates server machines in response to application events inferred from the system calls. From the programmer's perspective, all the machines running the application services they want to communicate with are always on (the machines are ``imaginary''), though in reality the cloud infrastructure upscales and downscales real machines for each service/application based on the information inferred from syscall interception. 
    \item We propose to implement this using Boxer?? \ana{Is that the plan?}
    \item \ana{This needs more thought...what exactly is the spectrum we want to discuss?} We also discuss the spectrum of approaches to unify the network-of-hosts VM-based application model and the serverless model of computation in the cloud. On one extreme, we can patch serverless frameworks to provide features that enable traditional off-the-shelf network-of-hosts applications to run. On the other extreme, we can design a new programming model that forces users to expose signals explicitly. Imaginary machines lies in the middle. 
\end{itemize}

\ana{End.}

